Network Localization Based Planning for Autonomous Underwater Vehicles with Inter-Vehicle Ranging

Localization between a swarm of AUVs can be entirely estimated through the use of range measurements between neighboring AUVs via a class of techniques commonly referred to as sensor network localization. However, the localization quality depends on network topology, with degenerate topologies, referred to as low-rigidity configurations, leading to ambiguous or highly uncertain localization results. This paper presents tools for rigidity-based analysis, planning, and control of a multi-AUV network which account for sensor noise and limited sensing range. We evaluate our long-term planning framework in several two-dimensional simulated environments and show we are able to generate paths in feasible time and guarantee a minimum network rigidity over the full course of the paths.

==> _region_.tex <==
\message{ !name(introduction.tex)}
\message{ !name(introduction.tex) !offset(5) }

\message{ !name(introduction.tex) !offset(-4) }


==> approach.tex <==
\section{Approach}
We seek to devise a time-scheduled path planning approach that returns a set of
paths which meet the predetermined rigidity constraints on network geometry. 

% Would it be better to ground the nodes which provide the 'fix'?
We define a quantitative notion of \textbf{network rigidity} for a given sensor
network as the 1st nontrivial eigenvalue of the rigidity matrix.
Trivial eigenvalues are all zero and correspond to the degrees of
freedom (DOF) of a coordinate system, two-dimensional space having 3-DOF.

We use this as a way of measuring how robust the network is to noise.

This minimum rigidity
serves as a tunable parameter, which allows for a tradeoff between robustness to
noise and ability to find a feasible set of trajectories.

From here our approach takes the form of priority-based multi-agent planning
on a graph, with the constraints that no two-agents are allowed to occupy the same
location at the same time and that the network rigidity must remain above the
pre-specified minimum rigidity at every timestep in the AUV trajectories.

To execute the priority planning we use a notion of validity for each AUV, where
each AUV is required to plan a path while occupying 

To reduce the amount of rigidity checking of possible configurations, we propose
several sets which are required




==> related_works.tex <==
\section{Related Works}

% Work on collaborative localization


% Work on formation control


% Work on multi-agent pathfinding


% % Work on sensor network localization
% AKA multidimensional scaling, graph realization, euclidean distance matrix
% completion, and sensor network localization

% Work on structural engineering




